Big Data Meets Telcos: A Proactive Caching Perspective

Mobile cellular networks are becoming increasingly complex to manage while classical deployment/optimization techniques and current solutions (i.e., cell densification, acquiring more spectrum, etc.) are cost-ineffective and thus seen as stopgaps. This calls for development of novel approaches that leverage recent advances in storage/memory, context-awareness, edge/cloud computing, and falls into framework of big data. However, the big data by itself is yet another complex phenomena to handle and comes with its notorious 4V: velocity, voracity, volume and variety. In this work, we address these issues in optimization of 5G wireless networks via the notion of proactive caching at the base stations. In particular, we investigate the gains of proactive caching in terms of backhaul offloadings and request satisfactions, while tackling the large-amount of available data for content popularity estimation. In order to estimate the content popularity, we first collect users' mobile traffic data from a Turkish telecom operator from several base stations in hours of time interval. Then, an analysis is carried out locally on a big data platform and the gains of proactive caching at the base stations are investigated via numerical simulations. It turns out that several gains are possible depending on the level of available information and storage size. For instance, with 10% of content ratings and 15.4 Gbyte of storage size (87% of total catalog size), proactive caching achieves 100% of request satisfaction and offloads 98% of the backhaul when considering 16 base stations.

==> figure-cumsize.tex <==
%%%%%%%%%%%%%%%%%%%%% Cumulative size of contents
\begin{figure}[!ht]
\centering
\begin{tikzpicture}
	\begin{axis}[
		width=0.80\columnwidth,
 		grid = major,
 		legend cell align=left,
 		xmode=log, 		
 		mark repeat={10},
% 		ymin=0,ymax=100,
 		legend style ={legend pos=north east},
 		xlabel={Cumulative Rank},
 		ylabel={Size [GByte]}]

 		%%%%% Cumulative size
 		\addplot+[blue!60!black, mark=o, mark size=1.8, thick]
 				  table [col sep=comma] {\string"results-globalpop-cumsize.csv"};
		 		  		
	\end{axis}
\end{tikzpicture}
\caption{Cumulative size of contents.}
\label{fig:globalpop-cumsize}%\vspace{-0.35cm}
\end{figure}
